Practicality of generalization guarantees for unsupervised domain adaptation with neural networks

Understanding generalization is crucial to confidently engineer and deploy machine learning models, especially when deployment implies a shift in the data domain. For such domain adaptation problems, we seek generalization bounds which are tractably computable and tight. If these desiderata can be reached, the bounds can serve as guarantees for adequate performance in deployment. However, in applications where deep neural networks are the models of choice, deriving results which fulfill these remains an unresolved challenge; most existing bounds are either vacuous or has non-estimable terms, even in favorable conditions. In this work, we evaluate existing bounds from the literature with potential to satisfy our desiderata on domain adaptation image classification tasks, where deep neural networks are preferred. We find that all bounds are vacuous and that sample generalization terms account for much of the observed looseness, especially when these terms interact with measures of domain shift. To overcome this and arrive at the tightest possible results, we combine each bound with recent data-dependent PAC-Bayes analysis, greatly improving the guarantees. We find that, when domain overlap can be assumed, a simple importance weighting extension of previous work provides the tightest estimable bound. Finally, we study which terms dominate the bounds and identify possible directions for further improvement.

==> reviewresponses.tex <==
Response to Reviewer vsaP:
We thank the reviewer for reviewing our work and their insightful comments. 

Concerning practicality of computation, we considered a restricted case where it is at least possible to accurately estimate the quantities in the bounds. The practicality of training a large number of models for this purpose depends on the size of the networks and the nature of the tasks. We have added a brief discussion of this in the limitation section of the Discussion.

We concur that the use of the PAC-Bayes bounds for model selection is an interesting topic. However, we found that investigating this in a more complete manner would have increased the amount of work substantially while not being directly related to the computation and comparison of the bounds, which is our primary focus. Therefore we chose to leave such an investigation to future work.

We agree with the reviewers points that assuming overlapping support is likely too strong of an assumption to be empirically viable and the assumption required for the MMD bound to hold is fairly opaque. The MMD assumption does not rely on overlap, but whether it is satisfied depends on the behavior of loss functions outside of the support of the labeled data. As such, it is not verifiable without overlap. If there is reason to believe that the function under estimation is smooth, the assumption is more plausible but should nevertheless be used with care. More work is needed to intuit for which tasks and models this is a reasonable assumption and when other ones are needed. We expanded the discussion on the intuition of overlap and the loss assumption in the discussion section. 

Response to Reviewer TMKi:
We thank the reviewer for their comments and helpful references to related work. The comments below are regarding the requested changes.

Regarding the importance weighting bound we have stated explicitly in section 3 that we assume that they are uniformly bounded and that we can calculate them exactly, based on knowledge of the data set construction, for simplicity.

We have added standard deviations to the bounds in figure 6 and similar figures in the appendix.

We thank the reviewer for reminding us of the works using localized discrepancies. We have added a discussion on these to the second section and a short note of the intractability of computing the discrepancy for a subset of promising classifiers when these are deep neural networks. This disqualifies them from consideration in this work as we study practically computable bounds.

Further on the point of lacking literature coverage. Paper [3] is primarily focused on achieving a bound which might be successfully minimised (in part) by methods like DANN. It thus uses a very specific construction which is unique in the sense that it requires a lot of assumptions on the structure of the domains under a representation mapping and how they are related. We have added a note at the end of section 2 exemplifying this as a direction for future work. However, we do not consider this work along with other representation learning approaches for reasons stated at the end of section 2. 

The last paper, [4], also focuses on constructions that can be effectively controlled by adversarial learning. We have added it to the overview section. However, the resulting bounds also contain the joint optimal error parameter $\lambda$ which disqualifies it similar to many other works considered in section 2.

Regarding the boundedness of the kernel. While we have not explicitly mentioned it in the paper, $K$ is bounded by 1 for our choice of kernel, the Gaussian RBF-kernel, irrespective of model. Hence, we can compute all parts of the bound.  However, making any concrete statement about the variation in tigher bounds on $K$ for neural networks is very hard. Generally speaking, the value might be high or low depending on the type of data considered, what kernel one chooses to work with etc. The kernel value itself is not directly influenced by the model choice, other than through the assumption that the loss can be pointwise bounded by a function in the RKHS given by $k$. 
 

Response to Reviewer iFWv:
We thank the reviewer for taking their time to review our work. We are glad to hear that the reviewer finds our extensions of previous work interesting. We share the sentiment. 

We have added a short introduction and definition of the MMD.

Concerning the effect of sample size. We have investigated the effect of simply increasing the amount of datapoints available when calculating which of course tightens the bounds. However, the question is what exactly increasing the sample means. If we constrain the total amount of datapoints, it is more difficult to disentangle effects as both the posterior learned and the bound calculation are affected. 

If the reviewer refers to just constraining the amount used for the bound it is simply a exercise of increasing $m$ in the bounds. This results in the IW and Add bounds becoming increasingly tight as they converge to the target risk. The Mult. and MMD bounds will still have the $\beta_\infty$ and $MMD$ terms respectively which will not allow them to become fully tight unless they are 1 and 0 respectively.




==> rewrite.tex <==
Main points to change
R1-----
- including the lacking literature aspects, i.e. bounds based on asymmetrically relaxed divergences, localization, and f-divergences. In particular, there should be a theoretical discussion on the tightness of such bounds. 

-since the experiments concern several seeds, including the deviation from the mean can be more informative on the behavior of the bounds. ### DONE, maybe comment on it somewhere, e.g. captions

-Either taking into account the estimation of importance weights, or clearly stating that it is assumed that they are known. ### DONE

-Stating that the importance weights are assumed to be uniformly bounded. ### DONE

-Adding a discussion on how K behaves for a neural network.
-------

Weaknesses:

R1-----
Some literature aspects of DA bounds are lacking, namely:
Asymmetrically relaxed discrepancies [3], where the importance weight is only required to be bounded in order to guarantee good adaptation, instead of requiring equality of distributions.
Localized discrepancies [1,2], where the restriction of the supremum defining the divergence to a proper subset of the hypothesis space yields significantly lower divergence measures as illustrated in [1].
Other important DA contributions with bounds leading to algorithms such as [4].
On importance weighting and the IW bound (Corollary 1):

- The IW bound proposed in the paper can become vacuous if . This can happen even if the source domain's support completely includes the target's. ### RESOLVED BY ADDITION BELOW
-In the IW bound, the estimation error of the weights is not taken into account, i.e. it assumes perfect computation of the importance weights . This goes against the spirit of the paper concerned with the tightness of generalization bounds. ### ADDED LINE IN SECTION 3 CLARIFYING THIS
-The MMD bound contains , a parameter of the kernel that controls the estimation error of the MMD. However, no discussion is provided on its behavior for neural networks, whereas a main motivation of the paper is the vacuity of classic generalization bounds in the case of neural networks, notably those relying on the VC dimension.
-------
Small edits:
R1-----
-In figure 5, a logarithmic scale figure for values close to the target error, and adding a grid, might facilitate reading. ### ADDED GRID

-In the discussion section, it is mentioned "The main obstacle for using existing bounds is that they ... ". I would say "computing" rather than "using", are such bounds are used to propose DA algorithms in several cases. ### CHANGED WORDING, although we maybe should change the whole sentence..
-------
